Dynamic Similarity Graph Construction with Kernel Density Estimation

In the kernel density estimation (KDE) problem, we are given a set $X$ of data points in $\mathbb{R}^d$, a kernel function $k: \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}$, and a query point $\mathbf{q} \in \mathbb{R}^d$, and the objective is to quickly output an estimate of $\sum_{\mathbf{x} \in X} k(\mathbf{q}, \mathbf{x})$. In this paper, we consider $\textsf{KDE}$ in the dynamic setting, and introduce a data structure that efficiently maintains the estimates for a set of query points as data points are added to $X$ over time. Based on this, we design a dynamic data structure that maintains a sparse approximation of the fully connected similarity graph on $X$, and develop a fast dynamic spectral clustering algorithm. We further evaluate the effectiveness of our algorithms on both synthetic and real-world datasets.

==> algorithms/spectral_clustering.tex <==
\begin{algorithm}[ht]
\caption{\textsf{SpectralClustering}}\label{alg:spectralclustering}
\KwData{$G=(V,E)$, $k\in\mathbb{N}$}
\KwResult{A partitioning $P_1, \ldots, P_k$}
Compute $f_1, \ldots, f_k$ of $\mathcal{L}_G$\; 
% \st{Initialize $j_{\mathrm{max}} \leftarrow \log_{C_d}{|\dmax|}$} \;
\For{$u \in V$}{
$F(u) \leftarrow \frac{1}{\sqrt{d_u}}\cdot (f_1(u),\ldots, f_k(u))^{\intercal}$\;
}
$P_1, \ldots, P_k \leftarrow k\mbox{-means} (\{F(u)\}_{u\in V}, k)$\;
\Return{$P_1, \ldots, P_k$}
\end{algorithm}

==> figures/dataset_info_table.tex <==
\begin{table}
  \caption{Dataset size information \label{tab:dataset-sizes}}
  \centering
  \begin{tabular}{lll}
    \toprule 
    Dataset & $n$ & $d$ \\
    \midrule
    blobs & 20,000 & 10 \\
    mnist & 70,000 & 728 \\
    cifar10 & 50,000 & 2,048 \\
    aloi & 108,000 & 128 \\
    msd & 515,345 & 90 \\
    covtype & 581,012 & 54 \\
    glove & 1,193,514 & 100 \\
    census & 2,458,285 & 68 \\
    \bottomrule
  \end{tabular}
\end{table}

==> figures/dynamic_kde_table.tex <==
\begin{table} [htb]
  \caption{}
  \label{tab:dynamic_kde}
  \centering
  \begin{tabular}{ccccccccc}
    \toprule
    & \multicolumn{2}{c}{Our Algorithm} & \multicolumn{2}{c}{CKNS} & \multicolumn{2}{c}{Dynamic RS} & \multicolumn{2}{c}{Exact}\\ 
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
    dataset & Time (s) & Err & Time (s) & Err & Time (s) & Err & Time (s) & Err\\ 
    \midrule
    shuttle &  20.4 &  0.157 &  42.2 &  0.147 & \textbf{ 3.2} &  0.076 &  12.3 & 0 \\
    mnist &  126.6 &  0.285 &  458.0 &  0.252 & \textbf{ 40.8} &  0.032 &  376.6 & 0 \\
    aloi &  74.6 &  0.143 &  343.2 &  0.048 & \textbf{ 36.5} &  0.011 &  195.6 & 0 \\
    msd & \textbf{ 306.4} &  0.388 &  14360.0 &  0.385 &  1887.8 &  5.430 &  2715.6 & 0 \\
    covtype & \textbf{ 210.1} &  0.202 &  2514.0 &  0.156 &  329.2 &  0.016 &  1869.6 & 0 \\
    glove & \textbf{ 631.0} &  0.061 &  4093.8 &  0.034 &  1015.9 &  0.000 &  5251.7 & 0 \\
    census & \textbf{ 814.2} &  0.112 &  10391.2 &  0.080 &  3422.2 &  0.005 &  16279.9 & 0 \\
    \bottomrule
  \end{tabular}
\end{table}

==> figures/dynamic_sg_table.tex <==
\begin{table} [htb]
  \caption{}
  \label{tab:dynamic_sg}
  \centering
  \begin{tabular}{ccccccc}
    \toprule
    & \multicolumn{3}{c}{Our Algorithm} & \multicolumn{3}{c}{FullyConnected} & \multicolumn{3}{c}{kNN}\\ 
    \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(lr){8-9}
    dataset & Time (s) & ARI & NMI & Time (s) & ARI & NMI & Time (s) & ARI & NMI\\ 
    \midrule
    mnist &  2405.0 &  0.200 &  0.509 & \textbf{ 106.2} &  0.984 &  0.959 &  8510.0 &  0.615 &  0.749 \\
    cifar10 &  1731.4 &  0.239 &  0.385 &  261.8 &  0.820 &  0.747 & \textbf{-1.0} & -1.000 & -1.000 \\
    \bottomrule
  \end{tabular}
\end{table}
